Characterizing Manipulation from AI Systems

Manipulation is a common concern in many domains, such as social media, advertising, and chatbots. As AI systems mediate more of our interactions with the world, it is important to understand the degree to which AI systems might manipulate humans without the intent of the system designers. Our work clarifies challenges in defining and measuring manipulation in the context of AI systems. Firstly, we build upon prior literature on manipulation from other fields and characterize the space of possible notions of manipulation, which we find to depend upon the concepts of incentives, intent, harm, and covertness. We review proposals on how to operationalize each factor. Second, we propose a definition of manipulation based on our characterization: a system is manipulative if it acts as if it were pursuing an incentive to change a human (or another agent) intentionally and covertly. Third, we discuss the connections between manipulation and related concepts, such as deception and coercion. Finally, we contextualize our operationalization of manipulation in some applications. Our overall assessment is that while some progress has been made in defining and measuring manipulation from AI systems, many gaps remain. In the absence of a consensus definition and reliable tools for measurement, we cannot rule out the possibility that AI systems learn to manipulate humans without the intent of the system designers. We argue that such manipulation poses a significant threat to human autonomy, suggesting that precautionary actions to mitigate it are warranted.

==> archived/order_relations.tex <==
%don't worry. maybe this section is just for my own enjoyment
\section{Order relations and preferences}

An foundational mathematics a relation $R$ is an operator which takes two arguments $a\in A$ $b\in B$ for sets $A$ and $B$ and evaluates to either True or False. By convention we write $aRb=True$ as $aRb$ and $aRb=False$ as $aRb$. The set of all positive answers can be thought of as a subset of the Cartesian product of $A$ and $B$. Normally relations are defined on the same set, that is to say $A=B$.

An order relation on set $A$ is one that has the following properties:

\begin{enumerate}
    \item \textbf{Reflexivity}: $aRa$ for $a$ in $A$ 
    \item \textbf{Anti-Symmetry}: If $aRb$ and $bRa$ then $a=b$ for $a,b\in A$
    \item \textbf{Transitivity}: If $aRb$ and $bRc$ then $aRc$ for $a,b,c \in A$
\end{enumerate}

An order relation $R$ on a set $A$ is total (aka linear) if any two elements in the set can be compared. 
An example of a total order relation on a set is the $\geq$ operator on the real numbers $\mathbb{R}$. Any attempt to translate preferences into real numbers via a utility function necessarily inherits these three properties. This is formalised by the Von Neumann-Morgenstern utility theorem. In this light, the four 'rationality' requirements that it makes (Completeness, Transitivity, Continuity and Independence) seem more like tools necessary to prove the theorem rather than deep statements about how preferences should work.

A partial-order relation on set $A$ is one where there exist $a,b \in A$ such that neither $aRb$ or $bRa$ is true. $A$ is said to be a partially ordered set or poset for short. Preference mappings to $\mathbb{R}^n$  for $n\geq2$ are posets (assuming there isn't some subsequent mapping onto $\mathbb{R}$). Typically we define an order relation $\leq$ as $(a,b)\leq (c,d)$ iff $a \leq c$ and $b\leq d$, for $a,b,c,d\in \mathbb{R}$. This means that certain pairs cannot be compared, for example in the  situations where $a<c$ and $b>d$ neither $(a,b)\leq(c,d)$ or $(c,d)\leq(a,b)$ is true.


